Predicting Visual Context for Unsupervised Event Segmentation in Continuous Photo-streams

Segmenting video content into events provides semantic structures for indexing, retrieval, and summarization. Since motion cues are not available in continuous photo-streams, and annotations in lifelogging are scarce and costly, the frames are usually clustered into events by comparing the visual features between them in an unsupervised way. However, such methodologies are ineffective to deal with heterogeneous events, e.g. taking a walk, and temporary changes in the sight direction, e.g. at a meeting. To address these limitations, we propose Contextual Event Segmentation (CES), a novel segmentation paradigm that uses an LSTM-based generative network to model the photo-stream sequences, predict their visual context, and track their evolution. CES decides whether a frame is an event boundary by comparing the visual context generated from the frames in the past, to the visual context predicted from the future. We implemented CES on a new and massive lifelogging dataset consisting of more than 1.5 million images spanning over 1,723 days. Experiments on the popular EDUB-Seg dataset show that our model outperforms the state-of-the-art by over 16% in f-measure. Furthermore, CES' performance is only 3 points below that of human annotators.

==> biblio.tex <==
%%% -*-BibTeX-*-
%%% Do NOT edit. File created by BibTeX with style
%%% ACM-Reference-Format-Journals [18-Jan-2012].

\begin{thebibliography}{43}

%%% ====================================================================
%%% NOTE TO THE USER: you can override these defaults by providing
%%% customized versions of any of these macros before the \bibliography
%%% command.  Each of them MUST provide its own final punctuation,
%%% except for \shownote{}, \showDOI{}, and \showURL{}.  The latter two
%%% do not use final punctuation, in order to avoid confusing it with
%%% the Web address.
%%%
%%% To suppress output of a particular field, define its macro to expand
%%% to an empty string, or better, \unskip, like this:
%%%
%%% \newcommand{\showDOI}[1]{\unskip}   % LaTeX syntax
%%%
%%% \def \showDOI #1{\unskip}           % plain TeX syntax
%%%
%%% ====================================================================

\ifx \showCODEN    \undefined \def \showCODEN     #1{\unskip}     \fi
\ifx \showDOI      \undefined \def \showDOI       #1{#1}\fi
\ifx \showISBNx    \undefined \def \showISBNx     #1{\unskip}     \fi
\ifx \showISBNxiii \undefined \def \showISBNxiii  #1{\unskip}     \fi
\ifx \showISSN     \undefined \def \showISSN      #1{\unskip}     \fi
\ifx \showLCCN     \undefined \def \showLCCN      #1{\unskip}     \fi
\ifx \shownote     \undefined \def \shownote      #1{#1}          \fi
\ifx \showarticletitle \undefined \def \showarticletitle #1{#1}   \fi
\ifx \showURL      \undefined \def \showURL       {\relax}        \fi
% The following commands are used for tagged output and should be
% invisible to TeX
\providecommand\bibfield[2]{#2}
\providecommand\bibinfo[2]{#2}
\providecommand\natexlab[1]{#1}
\providecommand\showeprint[2][]{arXiv:#2}

\bibitem[\protect\citeauthoryear{??}{Wor}{2010}]%
        {WordNet}
 \bibinfo{year}{2010}\natexlab{}.
\newblock \bibinfo{title}{WordNet. {Princeton University}}.
\newblock   (\bibinfo{year}{2010}).
\newblock
\urldef\tempurl%
\url{http://wordnet.princeton.edu}
\showURL{%
\tempurl}


\bibitem[\protect\citeauthoryear{Aizawa, Ishijima, and Shiina}{Aizawa
  et~al\mbox{.}}{2001}]%
        {AizSum01}
\bibfield{author}{\bibinfo{person}{Kiyoharu Aizawa}, \bibinfo{person}{Kenichiro
  Ishijima}, {and} \bibinfo{person}{Makoto Shiina}.}
  \bibinfo{year}{2001}\natexlab{}.
\newblock \showarticletitle{Summarizing wearable video}. In
  \bibinfo{booktitle}{\emph{International Conference on Image Processing}},
  Vol.~\bibinfo{volume}{3}. \bibinfo{publisher}{IEEE}
\newblock


\bibitem[\protect\citeauthoryear{Bettadapura, Castro, and Essa}{Bettadapura
  et~al\mbox{.}}{2016}]%
        {bettadapura2016picturesque}
\bibfield{author}{\bibinfo{person}{Vinay Bettadapura}, \bibinfo{person}{Daniel
  Castro}, {and} \bibinfo{person}{Irfan Essa}.}
  \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Discovering picturesque highlights from egocentric
  vacation videos}. In \bibinfo{booktitle}{\emph{IEEE Winter Conference on Applications of Computer
  Vision (WACV), 2016}}. IEEE, \bibinfo{pages}{1--9}.
\newblock


\bibitem[\protect\citeauthoryear{Bhatnagar, Singh, Arora, and
  Jawahar}{Bhatnagar et~al\mbox{.}}{2017}]%
        {bhatnagarunsupervised}
\bibfield{author}{\bibinfo{person}{Bharat~Lal Bhatnagar},
  \bibinfo{person}{Suriya Singh}, \bibinfo{person}{Chetan Arora}, {and}
  \bibinfo{person}{CV Jawahar}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Unsupervised Learning of Deep Feature
  Representation for Clustering Egocentric Actions}. In
  \bibinfo{booktitle}{\emph{Proceedings of the Twenty-Sixth International Joint
  Conference on Artificial Intelligence, {IJCAI-17}}}.
  \bibinfo{pages}{1447--1453}.
\newblock


\bibitem[\protect\citeauthoryear{Bolanos, Dimiccoli, and Radeva}{Bolanos
  et~al\mbox{.}}{2017}]%
        {BolanosSurv}
\bibfield{author}{\bibinfo{person}{Marc Bolanos}, \bibinfo{person}{Mariella
  Dimiccoli}, {and} \bibinfo{person}{Petia Radeva}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Toward storytelling from visual lifelogging: An
  overview}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Human-Machine Systems}}
  \bibinfo{volume}{47}, \bibinfo{number}{1} (\bibinfo{year}{2017}),
  \bibinfo{pages}{77--90}.
\newblock


\bibitem[\protect\citeauthoryear{Bolanos, Mestre, Talavera, Gir{\'o}-i Nieto,
  and Radeva}{Bolanos et~al\mbox{.}}{2015}]%
        {bolanos2015visual}
\bibfield{author}{\bibinfo{person}{Marc Bolanos}, \bibinfo{person}{Ricard
  Mestre}, \bibinfo{person}{Estefan{\'\i}a Talavera}, \bibinfo{person}{Xavier
  Gir{\'o}-i Nieto}, {and} \bibinfo{person}{Petia Radeva}.}
  \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{Visual summary of egocentric photostreams by
  representative keyframes}. In \bibinfo{booktitle}{\emph{IEEE International Conference on
  Multimedia and Expo Workshops}}. IEEE,
  \bibinfo{pages}{1--6}.
\newblock


\bibitem[\protect\citeauthoryear{Bola{\~n}os, Peris, Casacuberta, Soler, and
  Radeva}{Bola{\~n}os et~al\mbox{.}}{2018}]%
        {bolanos2018egocentric}
\bibfield{author}{\bibinfo{person}{Marc Bola{\~n}os},
  \bibinfo{person}{{\'A}lvaro Peris}, \bibinfo{person}{Francisco Casacuberta},
  \bibinfo{person}{Sergi Soler}, {and} \bibinfo{person}{Petia Radeva}.}
  \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Egocentric video description based on
  temporally-linked sequences}.
\newblock \bibinfo{journal}{\emph{Journal of Visual Communication and Image
  Representation}}  \bibinfo{volume}{50} (\bibinfo{year}{2018}),
  \bibinfo{pages}{205--216}.
\newblock


\bibitem[\protect\citeauthoryear{Dang-Nguyen, Piras, Riegler, Boato, Zhou, and
  Gurrin}{Dang-Nguyen et~al\mbox{.}}{2017}]%
        {LifeLogTask17_CLEF}
\bibfield{author}{\bibinfo{person}{Duc-Tien Dang-Nguyen}, \bibinfo{person}{Luca
  Piras}, \bibinfo{person}{Michael Riegler}, \bibinfo{person}{Giulia Boato},
  \bibinfo{person}{Liting Zhou}, {and} \bibinfo{person}{Cathal Gurrin}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{{Overview of ImageCLEFlifelog 2017: Lifelog
  Retrieval and Summarization}}. In \bibinfo{booktitle}{\emph{CLEF2017 Working
  Notes}}.
  \bibinfo{address}{Dublin, Ireland}.
\newblock


\bibitem[\protect\citeauthoryear{del Molino, Boix, Lim, and Tan}{del Molino
  et~al\mbox{.}}{2017a}]%
        {AVS}
\bibfield{author}{\bibinfo{person}{Ana~Garcia del Molino},
  \bibinfo{person}{Xavier Boix}, \bibinfo{person}{Joo-Hwee Lim}, {and}
  \bibinfo{person}{Ah-Hwee Tan}.} \bibinfo{year}{2017}\natexlab{a}.
\newblock \showarticletitle{Active Video Summarization: Customized Summaries
  via On-line Interaction with the User}. In \bibinfo{booktitle}{\emph{AAAI
  Conference on Artificial Intelligence}}. \bibinfo{pages}{4046--4052}.
\newblock


\bibitem[\protect\citeauthoryear{del Molino, Tan, Lim, and Tan}{del Molino
  et~al\mbox{.}}{2017b}]%
        {MySurvey}
\bibfield{author}{\bibinfo{person}{Ana~Garcia del Molino},
  \bibinfo{person}{Cheston Tan}, \bibinfo{person}{Joo-Hwee Lim}, {and}
  \bibinfo{person}{Ah-Hwee Tan}.} \bibinfo{year}{2017}\natexlab{b}.
\newblock \showarticletitle{Summarization of egocentric videos: A comprehensive
  survey}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Human-Machine Systems}}
  \bibinfo{volume}{47}, \bibinfo{number}{1} (\bibinfo{year}{2017}),
  \bibinfo{pages}{65--76}.
\newblock


\bibitem[\protect\citeauthoryear{Dimiccoli, Bola{\~n}os, Talavera, Aghaei,
  Nikolov, and Radeva}{Dimiccoli et~al\mbox{.}}{2017}]%
        {dimiccoli2017sr}
\bibfield{author}{\bibinfo{person}{Mariella Dimiccoli}, \bibinfo{person}{Marc
  Bola{\~n}os}, \bibinfo{person}{Estefania Talavera}, \bibinfo{person}{Maedeh
  Aghaei}, \bibinfo{person}{Stavri~G Nikolov}, {and} \bibinfo{person}{Petia
  Radeva}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{SR-clustering: Semantic regularized clustering for
  egocentric photo streams segmentation}.
\newblock \bibinfo{journal}{\emph{Computer Vision and Image Understanding}}
  \bibinfo{volume}{155} (\bibinfo{year}{2017}), \bibinfo{pages}{55--69}.
\newblock


\bibitem[\protect\citeauthoryear{Doherty, Ó~Conaire, Blighe, Smeaton, and
  O'Connor}{Doherty et~al\mbox{.}}{2008a}]%
        {DohertyRet08}
\bibfield{author}{\bibinfo{person}{Aiden~R Doherty}, \bibinfo{person}{Ciar\'{a}n
  \'{O}~Conaire}, \bibinfo{person}{Michael Blighe}, \bibinfo{person}{Alan~F
  Smeaton}, {and} \bibinfo{person}{Noel~E O'Connor}.}
  \bibinfo{year}{2008}\natexlab{a}.
\newblock \showarticletitle{Combining image descriptors to effectively retrieve
  events from visual lifelogs}. In \bibinfo{booktitle}{\emph{Proceedings of the
  1st ACM International Conference on Multimedia Information Retrieval}}.
  \bibinfo{publisher}{ACM}, \bibinfo{pages}{10--17}.
\newblock


\bibitem[\protect\citeauthoryear{Doherty, Byrne, Smeaton, Jones, and
  Hughes}{Doherty et~al\mbox{.}}{2008b}]%
        {DohertyLL08}
\bibfield{author}{\bibinfo{person}{Aiden~R Doherty}, \bibinfo{person}{Daragh
  Byrne}, \bibinfo{person}{Alan~F Smeaton}, \bibinfo{person}{Gareth~JF Jones},
  {and} \bibinfo{person}{Mark Hughes}.} \bibinfo{year}{2008}\natexlab{b}.
\newblock \showarticletitle{Investigating keyframe selection methods in the
  novel domain of passively captured visual lifelogs}. In
  \bibinfo{booktitle}{\emph{Proceedings of the 2008 International Conference on
  Content-based Image and Video Retrieval}}. ACM, \bibinfo{pages}{259--268}.
\newblock
\showISBNx{1605580708}


\bibitem[\protect\citeauthoryear{Fathi, Hodgins, and Rehg}{Fathi
  et~al\mbox{.}}{2012}]%
        {FathiDisney}
\bibfield{author}{\bibinfo{person}{Alireza Fathi}, \bibinfo{person}{Jessica~K
  Hodgins}, {and} \bibinfo{person}{James~M Rehg}.}
  \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{Social interactions: A first-person perspective}.
  In \bibinfo{booktitle}{\emph{Computer Vision and Pattern Recognition (CVPR),
  2012 IEEE Conference on}}. IEEE, \bibinfo{pages}{1226--1233}.
\newblock


\bibitem[\protect\citeauthoryear{Furnari, Battiato, and Farinella}{Furnari
  et~al\mbox{.}}{2018}]%
        {furnari2018personal}
\bibfield{author}{\bibinfo{person}{Antonino Furnari},
  \bibinfo{person}{Sebastiano Battiato}, {and} \bibinfo{person}{Giovanni~Maria
  Farinella}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Personal-location-based temporal segmentation of
  egocentric videos for lifelogging applications}.
\newblock \bibinfo{journal}{\emph{Journal of Visual Communication and Image
  Representation}}.
\newblock



\bibitem[\protect\citeauthoryear{Gal and Ghahramani}{Gal and
  Ghahramani}{2016}]%
        {gal2016theoretically}
\bibfield{author}{\bibinfo{person}{Yarin Gal} {and} \bibinfo{person}{Zoubin
  Ghahramani}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{A theoretically grounded application of dropout in
  recurrent neural networks}. In \bibinfo{booktitle}{\emph{Advances in Neural
  Information Processing Systems}}. \bibinfo{pages}{1019--1027}.
\newblock


\bibitem[\protect\citeauthoryear{Garcia~del Molino, Bappaditya, Lin, Lim,
  Vigneshwaran, and Vijay}{Garcia~del Molino et~al\mbox{.}}{2017}]%
        {I2R2017CLEF}
\bibfield{author}{\bibinfo{person}{Ana Garcia~del Molino},
  \bibinfo{person}{Mandal Bappaditya}, \bibinfo{person}{Jie Lin},
  \bibinfo{person}{Joo-Hwee Lim}, \bibinfo{person}{Subbaraju Vigneshwaran},
  {and} \bibinfo{person}{Chandrasekhar Vijay}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{{VC-I2R} at {ImageCLEF2017}: Ensemble of Deep
  Learned Features for Lifelog Video Summarization}. In
  \bibinfo{booktitle}{\emph{CLEF working notes, CEUR}}.
\newblock


\bibitem[\protect\citeauthoryear{Garc{\'\i}a~del Molino and
  Gygli}{Garc{\'\i}a~del Molino and Gygli}{2018}]%
        {GarciadelMolino2018phd}
\bibfield{author}{\bibinfo{person}{Ana Garc{\'\i}a~del Molino} {and}
  \bibinfo{person}{Michael Gygli}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{PHD-GIFs: Personalized Highlight Detection for
  Automatic GIF Creation}. In \bibinfo{booktitle}{\emph{Proceedings of the 2018
  ACM on Multimedia Conference}} \emph{(\bibinfo{series}{MM '18})}.
  \bibinfo{publisher}{ACM}, \bibinfo{address}{New York, NY, USA}.
\newblock


\bibitem[\protect\citeauthoryear{Gurrin, Joho, Hopfgartner, Zhou, Gupta,
  Albatal, Nguyen, and Tien}{Gurrin et~al\mbox{.}}{2017}]%
        {NTCIR_db}
\bibfield{author}{\bibinfo{person}{Cathal Gurrin}, \bibinfo{person}{Hideo
  Joho}, \bibinfo{person}{Frank Hopfgartner}, \bibinfo{person}{Liting Zhou},
  \bibinfo{person}{Rashmi Gupta}, \bibinfo{person}{Rami Albatal},
  \bibinfo{person}{Dang Nguyen}, {and} \bibinfo{person}{Duc Tien}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Overview of NTCIR-13 lifelog-2 task}.


\bibitem[\protect\citeauthoryear{Gygli, Grabner, Riemenschneider, and
  Van~Gool}{Gygli et~al\mbox{.}}{2014}]%
        {GygliSum14}
\bibfield{author}{\bibinfo{person}{Michael Gygli}, \bibinfo{person}{Helmut
  Grabner}, \bibinfo{person}{Hayko Riemenschneider}, {and} \bibinfo{person}{Luc
  Van~Gool}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{Creating summaries from user videos}.
\newblock In \bibinfo{booktitle}{\emph{Computer Vision--ECCV}}.
  \bibinfo{publisher}{Springer}.
\newblock


\bibitem[\protect\citeauthoryear{Harvey, Langheinrich, and Ward}{Harvey
  et~al\mbox{.}}{2016}]%
        {harvey2016remembering}
\bibfield{author}{\bibinfo{person}{Morgan Harvey}, \bibinfo{person}{Marc
  Langheinrich}, {and} \bibinfo{person}{Geoff Ward}.}
  \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Remembering through lifelogging: A survey of human
  memory augmentation}.
\newblock \bibinfo{journal}{\emph{Pervasive and Mobile Computing}}
  \bibinfo{volume}{27} (\bibinfo{year}{2016}), \bibinfo{pages}{14--26}.
\newblock


\bibitem[\protect\citeauthoryear{Healy, Gurrin, and Smeaton}{Healy
  et~al\mbox{.}}{2014}]%
        {EEG2014}
\bibfield{author}{\bibinfo{person}{Graham Healy}, \bibinfo{person}{Cathal
  Gurrin}, {and} \bibinfo{person}{Alan~F Smeaton}.}
  \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{Lifelogging and {EEG}: utilising neural signals for
  sorting lifelog image data}.
\newblock  (\bibinfo{year}{2014}).
\newblock


\bibitem[\protect\citeauthoryear{Hu, Xie, Li, Zeng, and Maybank}{Hu
  et~al\mbox{.}}{2011}]%
        {HuSurv}
\bibfield{author}{\bibinfo{person}{Weiming Hu}, \bibinfo{person}{Nianhua Xie},
  \bibinfo{person}{Li Li}, \bibinfo{person}{Xianglin Zeng}, {and}
  \bibinfo{person}{Stephen Maybank}.} \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{A survey on visual content-based video indexing and
  retrieval}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Systems, Man, and Cybernetics, Part C:
  Applications and Reviews}} \bibinfo{volume}{41},
  \bibinfo{number}{6} (\bibinfo{year}{2011}).
\newblock


\bibitem[\protect\citeauthoryear{Lee, Ghosh, and Grauman}{Lee
  et~al\mbox{.}}{2012}]%
        {LeeDisco12}
\bibfield{author}{\bibinfo{person}{Yong~Jae Lee}, \bibinfo{person}{Joydeep
  Ghosh}, {and} \bibinfo{person}{Kristen Grauman}.}
  \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{Discovering important people and objects for
  egocentric video summarization.}. In \bibinfo{booktitle}{\emph{Computer
  Vision and Pattern Recognition}}, Vol.~\bibinfo{volume}{2}.
  \bibinfo{pages}{6}.
\newblock


\bibitem[\protect\citeauthoryear{Lee and Grauman}{Lee and Grauman}{2015}]%
        {LeePred15}
\bibfield{author}{\bibinfo{person}{Yong~Jae Lee} {and} \bibinfo{person}{Kristen
  Grauman}.} \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{Predicting important objects for egocentric video
  summarization}.
\newblock \bibinfo{journal}{\emph{International Journal of Computer Vision}}
  (\bibinfo{year}{2015}).
\newblock


\bibitem[\protect\citeauthoryear{Lin, Garcia~del Molino, Xu, Fang,
  Vigneshwaran, and Lim}{Lin et~al\mbox{.}}{2017}]%
        {I2R2017NTCIR}
\bibfield{author}{\bibinfo{person}{Jie Lin}, \bibinfo{person}{Ana Garcia~del
  Molino}, \bibinfo{person}{Qianli Xu}, \bibinfo{person}{Fen Fang},
  \bibinfo{person}{Subbaraju Vigneshwaran}, {and} \bibinfo{person}{Joo-Hwee
  Lim}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{{VC-I2R} at the {NTCIR-13} Lifelog Semantic Access
  Task}. In \bibinfo{booktitle}{\emph{Proceedings of NTCIR-13, Tokyo, Japan}}.
\newblock


\bibitem[\protect\citeauthoryear{Lin and Hauptmann}{Lin and Hauptmann}{2006}]%
        {lin2006structuring}
\bibfield{author}{\bibinfo{person}{Wei-Hao Lin} {and}
  \bibinfo{person}{Alexander Hauptmann}.} \bibinfo{year}{2006}\natexlab{}.
\newblock \showarticletitle{Structuring continuous video recordings of everyday
  life using time-constrained clustering}. In
  \bibinfo{booktitle}{\emph{Multimedia Content Analysis, Management, and
  Retrieval 2006}}, Vol.~\bibinfo{volume}{6073}. International Society for
  Optics and Photonics, \bibinfo{pages}{60730D}.
\newblock


\bibitem[\protect\citeauthoryear{Liu, Fu, Mei, and Chen}{Liu
  et~al\mbox{.}}{2017}]%
        {liu2017let}
\bibfield{author}{\bibinfo{person}{Yu Liu}, \bibinfo{person}{Jianlong Fu},
  \bibinfo{person}{Tao Mei}, {and} \bibinfo{person}{Chang~Wen Chen}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \bibinfo{title}{Let Your Photos Talk: Generating Narrative Paragraph
  for Photo Stream via Bidirectional Attention Recurrent Neural Networks}.
\newblock   (\bibinfo{year}{2017}).
\newblock


\bibitem[\protect\citeauthoryear{Lu and Grauman}{Lu and Grauman}{2013}]%
        {LuSD}
\bibfield{author}{\bibinfo{person}{Zheng Lu} {and} \bibinfo{person}{Kristen
  Grauman}.} \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{Story-driven summarization for egocentric video}.
  In \bibinfo{booktitle}{\emph{Computer Vision and Pattern Recognition}}.
  \bibinfo{publisher}{IEEE}, \bibinfo{pages}{2714--2721}.
\newblock


\bibitem[\protect\citeauthoryear{Money and Agius}{Money and Agius}{2008}]%
        {MoneySurv}
\bibfield{author}{\bibinfo{person}{Arthur~G Money} {and} \bibinfo{person}{Harry
  Agius}.} \bibinfo{year}{2008}\natexlab{}.
\newblock \showarticletitle{Video summarisation: A conceptual framework and
  survey of the state of the art}.
\newblock \bibinfo{journal}{\emph{Journal of Visual Communication and Image
  Representation}} \bibinfo{volume}{19}, \bibinfo{number}{2}
  (\bibinfo{year}{2008}), \bibinfo{pages}{121--143}.
\newblock


\bibitem[\protect\citeauthoryear{Ng, Sawahata, and Aizawa}{Ng
  et~al\mbox{.}}{2002}]%
        {NgSum}
\bibfield{author}{\bibinfo{person}{Hamg~Wei Ng}, \bibinfo{person}{Yasuhito
  Sawahata}, {and} \bibinfo{person}{Kiyoharu Aizawa}.}
  \bibinfo{year}{2002}\natexlab{}.
\newblock \showarticletitle{Summarization of wearable videos using support
  vector machine}. In \bibinfo{booktitle}{\emph{International Conference on
  Multimedia and Expo}}, Vol.~\bibinfo{volume}{1}. IEEE,
  \bibinfo{pages}{325--328}.
\newblock
\showISBNx{0780373049}


\bibitem[\protect\citeauthoryear{Poleg, Arora, and Peleg}{Poleg
  et~al\mbox{.}}{2014}]%
        {PolegSeg}
\bibfield{author}{\bibinfo{person}{Yair Poleg}, \bibinfo{person}{Chetan Arora},
  {and} \bibinfo{person}{Shmuel Peleg}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{Temporal segmentation of egocentric videos}. In
  \bibinfo{booktitle}{\emph{Proceedings of the IEEE Conference on Computer
  Vision and Pattern Recognition}}. \bibinfo{pages}{2537--2544}.
\newblock


\bibitem[\protect\citeauthoryear{Poleg, Ephrat, Peleg, and Arora}{Poleg
  et~al\mbox{.}}{2016}]%
        {PolegCNN}
\bibfield{author}{\bibinfo{person}{Yair Poleg}, \bibinfo{person}{Ariel Ephrat},
  \bibinfo{person}{Shmuel Peleg}, {and} \bibinfo{person}{Chetan Arora}.}
  \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Compact cnn for indexing egocentric videos}. In
  \bibinfo{booktitle}{\emph{Applications of Computer Vision (WACV), 2016 IEEE
  Winter Conference on}}. IEEE, \bibinfo{pages}{1--9}.
\newblock


\bibitem[\protect\citeauthoryear{Potapov, Douze, Harchaoui, and Schmid}{Potapov
  et~al\mbox{.}}{2014}]%
        {PotapovSum}
\bibfield{author}{\bibinfo{person}{Danila Potapov}, \bibinfo{person}{Matthijs
  Douze}, \bibinfo{person}{Zaid Harchaoui}, {and} \bibinfo{person}{Cordelia
  Schmid}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{Category-specific video summarization}.
\newblock \bibinfo{journal}{\emph{Computer Vision--ECCV}}
  (\bibinfo{year}{2014}), \bibinfo{pages}{540--555}.
\newblock


\bibitem[\protect\citeauthoryear{Spriggs, De~La~Torre, and Hebert}{Spriggs
  et~al\mbox{.}}{2009}]%
        {spriggs2009temporal}
\bibfield{author}{\bibinfo{person}{Ekaterina~H Spriggs},
  \bibinfo{person}{Fernando De~La~Torre}, {and} \bibinfo{person}{Martial
  Hebert}.} \bibinfo{year}{2009}\natexlab{}.
\newblock \showarticletitle{Temporal segmentation and activity classification
  from first-person sensing}. In \bibinfo{booktitle}{\emph{Computer Vision and
  Pattern Recognition Workshops, 2009}}. IEEE, \bibinfo{pages}{17--24}.
\newblock


\bibitem[\protect\citeauthoryear{Srivastava, Mansimov, and
  Salakhudinov}{Srivastava et~al\mbox{.}}{2015}]%
        {srivastava2015unsupervised}
\bibfield{author}{\bibinfo{person}{Nitish Srivastava}, \bibinfo{person}{Elman
  Mansimov}, {and} \bibinfo{person}{Ruslan Salakhudinov}.}
  \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{Unsupervised learning of video representations
  using {LSTMs}}. In \bibinfo{booktitle}{\emph{International Conference on
  Machine Learning}}. \bibinfo{pages}{843--852}.
\newblock


\bibitem[\protect\citeauthoryear{Szegedy, Vanhoucke, Ioffe, Shlens, and
  Wojna}{Szegedy et~al\mbox{.}}{2016}]%
        {szegedy2016rethinking}
\bibfield{author}{\bibinfo{person}{Christian Szegedy}, \bibinfo{person}{Vincent
  Vanhoucke}, \bibinfo{person}{Sergey Ioffe}, \bibinfo{person}{Jon Shlens},
  {and} \bibinfo{person}{Zbigniew Wojna}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Rethinking the inception architecture for computer
  vision}. In \bibinfo{booktitle}{\emph{Proceedings of the IEEE Conference on
  Computer Vision and Pattern Recognition}}.
\newblock


\bibitem[\protect\citeauthoryear{Varini, Serra, and Cucchiara}{Varini
  et~al\mbox{.}}{2015}]%
        {VariniPref}
\bibfield{author}{\bibinfo{person}{Patrizia Varini}, \bibinfo{person}{Giuseppe
  Serra}, {and} \bibinfo{person}{Rita Cucchiara}.}
  \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{Egocentric Video Summarization of Cultural Tour
  Based on User Preferences}. In \bibinfo{booktitle}{\emph{Proceedings of the
  23rd Annual ACM Conference on Multimedia Conference}}.
  \bibinfo{publisher}{ACM}, \bibinfo{pages}{931--934}.
\newblock


\bibitem[\protect\citeauthoryear{Xiong and Grauman}{Xiong and Grauman}{2014}]%
        {XiongSnap}
\bibfield{author}{\bibinfo{person}{Bo Xiong} {and} \bibinfo{person}{Kristen
  Grauman}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{Detecting snap points in egocentric video with a
  web photo prior}.
\newblock \bibinfo{journal}{\emph{Computer Vision--ECCV}}
  (\bibinfo{year}{2014}), \bibinfo{pages}{282--298}.
\newblock


\bibitem[\protect\citeauthoryear{Xu, Mukherjee, Li, Warner, Rehg, and Singh}{Xu
  et~al\mbox{.}}{2015}]%
        {XuGaze}
\bibfield{author}{\bibinfo{person}{Jia Xu}, \bibinfo{person}{Lopamudra
  Mukherjee}, \bibinfo{person}{Yin Li}, \bibinfo{person}{Jamieson Warner},
  \bibinfo{person}{James~M Rehg}, {and} \bibinfo{person}{Vikas Singh}.}
  \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{Gaze-Enabled Egocentric Video Summarization via
  Constrained Submodular Maximization}. In
  \bibinfo{booktitle}{\emph{Proceedings of the IEEE Conference on Computer
  Vision and Pattern Recognition}}. \bibinfo{pages}{2235--2244}.
\newblock


\bibitem[\protect\citeauthoryear{Yamamoto, Nishimura, Akagi, Takimoto, Inoue,
  and Toda}{Yamamoto et~al\mbox{.}}{2017}]%
        {yamamoto2017pbg}
\bibfield{author}{\bibinfo{person}{Shuhei Yamamoto}, \bibinfo{person}{Takuya
  Nishimura}, \bibinfo{person}{Yasunori Akagi}, \bibinfo{person}{Yoshiaki
  Takimoto}, \bibinfo{person}{Takafumi Inoue}, {and} \bibinfo{person}{Hiroyuki
  Toda}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Pbg at the ntcir-13 lifelog-2 lat, lsat, and lest
  tasks}.
\newblock \bibinfo{journal}{\emph{Proceedings of NTCIR-13, Tokyo, Japan}}
  (\bibinfo{year}{2017}).
\newblock


\bibitem[\protect\citeauthoryear{Yu, Bansal, and Berg}{Yu
  et~al\mbox{.}}{2017}]%
        {yu2017hierarchically}
\bibfield{author}{\bibinfo{person}{Licheng Yu}, \bibinfo{person}{Mohit Bansal},
  {and} \bibinfo{person}{Tamara~L Berg}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Hierarchically-Attentive RNN for Album
  Summarization and Storytelling}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:1708.02977}}.
\newblock


\bibitem[\protect\citeauthoryear{Zaki, Meira~Jr, and Meira}{Zaki
  et~al\mbox{.}}{2014}]%
        {zaki2014data}
\bibfield{author}{\bibinfo{person}{Mohammed~J Zaki}, \bibinfo{person}{Wagner
  Meira~Jr}, {and} \bibinfo{person}{Wagner Meira}.}
  \bibinfo{year}{2014}\natexlab{}.
\newblock \bibinfo{booktitle}{\emph{Data mining and analysis: fundamental
  concepts and algorithms}}.
\newblock \bibinfo{publisher}{Cambridge University Press}.
\newblock


\end{thebibliography}


==> deprecated.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/prediction.pdf}%{Figures.pdf}
	\vspace*{-2pt}
	\caption{An example of the prediction signal. We can observe that the formulation is very consistent with the ground truth. The few cases in which the prediction fails are usually due to long occlusions or short events within the same space.}
	\label{fig:prediction}
\end{figure}

%+++++++++++++++++++++++++++++++++++++++++++++++++++++%


\subsection{Datasets}
Three different sources are used to collect the images for the experiments. All of them are recorded with the Narrative Clip camera:

\textbf{R3:} we introduce in this paper a new dataset for lifelogging analysis. It consists of more than $1,4$ million images, captured in an unconstrained manner by $57$ users during a total of $1723$ days. $80\%$ of this dataset is used to train the sequence to sequence model. The other $20\%$ is kept for testing of that model.

\textbf{CLEF~\cite{LifeLogTask17_CLEF} and NTCIR~\cite{I2R2017NTCIR}:} this joined dataset consists of about $125,000$ images captured by $5$ users over the course of $170$ days. As with R3, we use $20\%$ of these datasets to train the sequence to sequence model, and $80\%$ to test it.

% \textbf{EDUB-SegDesc~\cite{bolanos2018egocentric} and EDUB-Seg~\cite{dimiccoli2017sr}:} these two datasets are annotated with the event boundary locations. We use EDUB-SegDesc (which consists of XXXX images captured by 11 users over 50 days) as validation data, and EDUB-Seg (XXX images for 7 users and 20 days) to test the model. This way, we can compare against the state of the art easily.
 \textbf{EDUB-Seg~\cite{dimiccoli2017sr}:} this dataset is annotated with the event boundary locations. It consists of around $15,000$ images captured by $7$ users during $20$ days. The semantic features for $12$ of the lifelogs are also available. Therefore, we compare our method to the baselines in two overlapping sets of this dataset.
 
 
 \subsection{Event boundary candidates}
\subsubsection{Unsupervised Event Segmentation}
To differentiate local outliers from actual event boundaries in an unsupervised manner, the future prediction error and the past prediction error are substracted. \todo{[blablabla]}
\subsubsection{Supervised Event Segmentation}
biLSTM fed with prediction error for future sequence of $N$ frames and sequence embedding representation at $t-1$ (see Fig. \ref{fig:dl}). \todo{[blablabla]}

\subsection{Pruning of event boundary candidates}
Feature distances between consecutive events, and compactness of the events with and without that boundary can be used to fine tune the boundary prediction. To prevent noise from bad event segmentation, the 15 frames before/after the boundary are considered to form the event, disregarding any additional frame in the event, or additional boundaries in between.
\subsubsection{Supervised Pruning}
An SVM is trained using both distances between events (\ie for boundary $k$, $d(e_k, e_{k+1})$, compactness of the events wraping the boundary $e_i$ and $e_{k+1}$, and compactness of the union of both events, $e_k \cup e_{k+1}$. \todo{[blablabla]}


%----------------------------------------------------------------------------------%
\begin{algorithm}[t!]
 \caption{\small Overview of the proposed method}
 \label{al:Alg}
 \small
\emph{$\triangleright$ Get expectation and prediction error:}\\
 $\hat{\mathbf{xf}}(t) = [\hat{\mathbf{x}}_k | t \leq k < t + M] \leftarrow $ predicted from  $[\mathbf{x}_k | t - N \leq k < t]$\\
 
 $\hat{\mathbf{xp}}(t) = [\hat{\mathbf{x}}_k | t \geq  k > t - M]\leftarrow $ predicted from $[\mathbf{x}_k | t+N \geq k > t]$\\
 
%  $ef(t) = [mse(\hat{\mathbf{xf}}_k - \mathbf{x}_k)]_{\forall t \leq k < t + N}$\\
%  $ep(t) = [mse(\hat{\mathbf{xp}}_k - \mathbf{x}_k)]_{\forall t \geq  k > t - N}$
$ef(t) = mean(mse(\hat{\mathbf{xf}}(t), \mathbf{xf}(t)))$\\
$ep(t) = mean(mse(\hat{\mathbf{xp}}(t), \mathbf{xf}(t)))$\\
\hrulefill \\
\emph{$\triangleright$ Detect boundary candidates:}\\
\eIf{{unsupervised}}{
      $pred = abs(ef - ep)$
      }{$pred\leftarrow$ biLSTM output given $ef, ep$}
$b = \{t \,  | \, (\dfrac{\delta pred}{\delta t} == 0 )\}$ \\
\hrulefill \\
\emph{$\triangleright$ Prune boundary candidates:}\\
$e_k = \{frame_i\}_{b_k \leq i < b_{k+1}}, \forall b$ \\
\eIf{{unsupervised}}{
$d(k) = dist(e_k, e_{k+1})$\\ 
$b = \{b_k | d(k) \geq mean(d) \} $}
{
$d(k) = [dist(e_k, e_{k+1}), comp(e_k), comp(e_{k+1}), comp(e_k \cup e_{k+1})]$\\ 
$w \leftarrow $ trained with SVM \\ 
$b = \{b_k | d(k)*w > .5 \} $}
\end{algorithm}

%----------------------------------------------------------------------------------%


%----------------------------------------------------------------------------------%

\begin{figure*}[t]
\centering
%\setlength\extrarowheight{1ex}
\setlength{\tabcolsep}{1pt}
\begin{tabular}[width=\textwidth]{@{}c@{}c@{}cc@{}c@{}ccc@{}c@{}cc@{}c@{}c}
\includegraphics[width=.08\linewidth]{figures/TP/fig0.jpg} %&\includegraphics[width=.08\linewidth]{figures/TP/fig1.jpg}
&\includegraphics[width=.08\linewidth]{figures/TP/fig2.jpg}&\includegraphics[width=.08\linewidth]{figures/TP/fig3.jpg}
&\includegraphics[width=.08\linewidth]{figures/TP/fig4.jpg}&\includegraphics[width=.08\linewidth]{figures/TP/fig5.jpg}&\includegraphics[width=.08\linewidth]{figures/TP/fig6.jpg}&
&
\includegraphics[width=.08\linewidth]{figures/FP/fig0.jpg} &\includegraphics[width=.08\linewidth]{figures/FP/fig1.jpg}
&\includegraphics[width=.08\linewidth]{figures/FP/fig2.jpg}%\includegraphics[width=.08\linewidth]{figures/FP/fig3.jpg}&
&\includegraphics[width=.08\linewidth]{figures/FP/fig4.jpg}&\includegraphics[width=.08\linewidth]{figures/FP/fig5.jpg}&\includegraphics[width=.08\linewidth]{figures/FP/fig6.jpg} \\
\multicolumn{6}{@{}c@{}}{(a) TP}&&\multicolumn{6}{@{}c@{}}{(b) FP}\\
\includegraphics[width=.08\linewidth]{figures/TN/fig0.jpg} &\includegraphics[width=.08\linewidth]{figures/TN/fig1.jpg}
&\includegraphics[width=.08\linewidth]{figures/TN/fig2.jpg}&\includegraphics[width=.08\linewidth]{figures/TN/fig3.jpg}
&\includegraphics[width=.08\linewidth]{figures/TN/fig4.jpg}&%\includegraphics[width=.08\linewidth]{figures/TN/fig5.jpg}&
\includegraphics[width=.08\linewidth]{figures/TN/fig6.jpg}&
&
%\includegraphics[width=.08\linewidth]{figures/FN/fig0.jpg} &
\includegraphics[width=.08\linewidth]{figures/FN/fig1.jpg}&\includegraphics[width=.08\linewidth]{figures/FN/fig2.jpg}&\includegraphics[width=.08\linewidth]{figures/FN/fig3.jpg}
&\includegraphics[width=.08\linewidth]{figures/FN/fig4.jpg}&\includegraphics[width=.08\linewidth]{figures/FN/fig5.jpg}&\includegraphics[width=.08\linewidth]{figures/FN/fig6.jpg}
\\
\multicolumn{6}{@{}c@{}}{(c) TN}&&\multicolumn{6}{@{}c@{}}{(d) FN}
\end{tabular}
\caption{Qualitative examples. SES performs better than the baselines for boundaries that separate heterogeneous events (a), and events with different points of view (c). That, however, may be misleading when the boundary between two different activities falls within the same physical space (d), or when an occlusion spans many frames (b).}
\label{fig:examples}
\end{figure*}

%----------------------------------------------------------------------------------%



\begin{table}[t!]
\centering
\setlength\extrarowheight{.2ex}
\setlength{\tabcolsep}{3pt}
\begin{tabular}[width=\textwidth]{@{}l|ccc|ccc}
\multicolumn{1}{@{}c@{}}{}& \multicolumn{3}{@{}c@{}}{EDUB-Seg12}  &  \multicolumn{3}{@{}c@{}}{EDUB-Seg20}\\
\multicolumn{1}{@{}c@{}|}{method} & F1  & Prec. & Rec. & F1 & Prec. & Rec. \\ \hline

k-means smoothed & .51 & .39 & .81 & .51 & .39 & .82\\
% w/SVM: Small set:[0.50869127, 0.39223224, 0.81495218] Full set:[0.51387895, 0.38994595, 0.82006465]

AC-Color~\cite{LeePred15} &  .36 & .23 & .91 & .38 & .25 & .90 \\
%../SR-Clustering/ResultsSR/ResultsKG/ small_set [ 0.56598025  0.46552649  0.32099105  0.94224537] / full_set [ 0.55900571  0.46694801  0.32081414  0.9237951 ]
%../SR-Clustering/ResultsSR/ResultsKGunsmoothed60/ small_set [ 0.62801424  0.3622317   0.23345957  0.9081858 ]/ full_set [ 0.63114073  0.38185665  0.24797759  0.90021879]

SR-ClusteringCNN~\cite{dimiccoli2017sr}& .50 & .70 & .47 & .53 & .68 & .49\\
SR-ClusteringImagga~\cite{dimiccoli2017sr} & .53 & .50 & .62 & &-&\\
KTS~\cite{PotapovSum}& .50 & .36 & .93 & .53 & .40 & .87\\[.7ex] \hline 
%KTS_segmentation/ small_set [0.60847789 0.49720712 0.35763027 0.93298611] / full_set [0.61445518 0.5256289  0.39683623 0.86708138]
%error (prev./next frame) &  0.44 & 0.33 & 0.81 & 0.43 & 0.31 & 0.81\\%test_config(5, [0, 0], dist=do_nothing, sup=False, no_expectation=True)
SES-error (local max) & 0.49 & 0.38 & 0.82 & 0.47 & 0.36 & 0.81\\%test_config(5, [0, 0], dist=do_nothing, sup=False) True first_error,do_nothing,5,0.00_0.00,do_nothing [0.50925843 0.45393935 0.32765996 0.83450355]
SES-emb (local max) & 0.70 & 0.66 & 0.80 & 0.67 & 0.63 & 0.76\\ %diff_embedding_cos,do_nothing,5,-1.00_0.00,do_nothing
model56c10 & 0.70 & 0.66 & 0.80 & 0.67 & 0.63 & 0.76\\ %TruePred_TrueCond_10_RMSprop0.0005_0_56c10
modeld33b3 & 0.70 & 0.66 & 0.80 & 0.69 & 0.65 & 0.77\\ %True diff_embedding_cos,do_nothing,5,-1.00_0.00,do_nothing, TruePred_TrueCond_1024_RMSprop0.0005_0_d33b3

model99581 & 0.70 & 0.67 & 0.79 & 0.69 & 0.65 & 0.77\\ %diff_embedding_cos,do_nothing,5,-1.00_0.00,do_nothing, TruePred_TrueCond_1024_N30_RMSprop0.0005_0.0_99581
model69c2a & 0.68 & 0.66 & 0.78 & 0.67 & 0.65 & 0.75\\ %diff_embedding_cos,do_nothing,5,-1.00_0.00,do_nothing , TruePred_TrueCond_1024_N100_RMSprop0.0005_0.0_69c2a
model38f03 & 0.69 & 0.65 & 0.80 & 0.67 & 0.63 & 0.75 \\%diff_embedding_cos,do_nothing,5,-1.00_0.00,do_nothing, TruePred_TrueCond_512_1_100_RMSprop0.000125_0_38f03


%embedding increment (local max) & 0.63 & 0.53 & 0.84 & 0.60 & 0.51 & 0.78\\
%averaged_embedding_do_nothing_5_0.00_0.25_do_nothing/ small_set [0.72703063 0.6268027  0.53345805 0.83544719]/ full_set [0.68968104 0.59772481 0.51158548 0.77879743]

% error w/ dist pruning & 0.60 & 0.54 & 0.76 & 0.60 & 0.52 & 0.76\\
% %True first_error,do_nothing,5,0.00_0.70,median_to_min_correlation & 0.65 & 0.64 & 0.71 & 0.62 & 0.63 & 0.66
% %first_error,do_nothing,5,0.00_-1.00,median_to_min_correlation & 0.60 & 0.54 & 0.76 & 0.60 & 0.52 & 0.76
% \hline\hline
% k-means w/ SVM * & 0.69 & 0.71 & 0.70 & 0.67 & 0.70 & 0.67\\ \hline
% error w/ svm pruning *  & 0.71 & 0.72 & 0.75 & 0.68 & 0.70 & 0.69\\ %test_config(5, [0, .5], error=first_error, norm=do_nothing, dist=linearSVM, sup=False) 
% %True averaged_embedding,do_nothing,5,0.00_0.50,linearSVM & 0.66 & 0.69 & 0.67 & 0.63 & 0.67 & 0.62
% % True first_error,do_nothing,4,0.00_0.50,linearSVM & 0.69 & 0.66 & 0.78 & 0.68 & 0.64 & 0.75
% % False first_error,do_nothing,4,0.00_0.50,rbfSVM [0.71654627 0.63201824 0.63651796 0.65231663]
% % True first_error,do_nothing,4,0.00_0.50,polySVM [0.74387525 0.65392267 0.66159274 0.68914135]
% % True first_error,do_nothing,5,0.00_0.50,linearSVM & 0.68 & 0.72 & 0.69 & 0.66 & 0.70 & 0.66
% diff emb w/SVM & 0.74 & 0.76 & 0.76 & 0.71 & 0.74 & 0.72 \\% diff_embedding_cos,do_nothing,5,0.00_0.50,polySVM
% biLSTM (local max) * & 0.51 & 0.59 & 0.55 & 0.48 & 0.58 & 0.49\\ %test_config(5, [0, 1], dist=do_nothing, sup=True) [0.50982655 0.4466046  0.33093783 0.79564858]
% % model110 [0.5973241  0.54772684 0.69505683 0.47810552] 0.49 & 0.41 & 0.72 0.49 & 0.39 & 0.73 
% % PredictorEmb_LateError_LSTM64_MLP8_RMSprop0.0041_0.0_ValSz0_c378e 0.46 & 0.36 & 0.76 0.48 & 0.36 & 0.78
% % PredictorError_LSTM16_MLP8_RMSprop0.0033_0.0_ValSz0_31f1e (5, [0, 1]) 0.49 & 0.38 & 0.80 0.48 & 0.37 & 0.80
% % Supervised /home/ana/models/PredictorEmb_LateError_LSTM64_MLP8_RMSprop0.01_0.0_ValSz0_f60a9: do_nothing,5,-0.50_1,do_nothing & 0.51 & 0.59 & 0.55 & 0.48 & 0.58 & 0.49
% biLSTM w/ svm pruning * & 0.67 & 0.74 & 0.65 & 0.65 & 0.72 & 0.62\\ %test_config(3, [0, 1], dist=polySVM, sup=True) /home/ana/models/PredictorEmb_LateError_LSTM64_MLP8_RMSprop0.01_0.0_ValSz0_f60a9
% %Supervised: do_nothing,4,0.00_1,linearSVM & 0.67 & 0.74 & 0.65 & 0.65 & 0.72 & 0.62
\hline
SES-emb w/ SVM pruning* & 0.74 & 0.76 & 0.76 & 0.71 & 0.74 & 0.72\\ 
%diff_embedding_cos,do_nothing,5,0.00_0.50,polySVM & 0.74 & 0.76 & 0.76 & 0.71 & 0.74 & 0.72
\end{tabular}
\caption{Results (F-measure, Precision and Recall) on the subset of $12$ lifelogs with available semantic tags and on the full EDUB-Seg.\\(*) Supervised pruning for reference purposes.}
\label{tab:results}
\end{table}


%-------------------------------------------------------------%
